A Holomorphic Embedding Based Continuation Method for Identifying Multiple Power Flow Solutions

In this paper, we propose an efficient continuation method for locating multiple power flow solutions. We adopt the holomorphic embedding technique to represent solution curves as holomorphic functions in the complex plane. The holomorphicity, which provides global information of the curve at any regular point, enables large step sizes in the path-following procedure such that non-singular curve segments can be traversed with very few steps. When approaching singular points, we switch to the traditional predictor-corrector routine to pass through them and switch back afterward to the holomorphic embedding routine. We also propose a warm starter when switching to the predictor-corrector routine, i.e. a large initial step size based on the poles of the Pad\'{e} approximation of the derived holomorphic function, since these poles reveal the locations of singularities on the curve. Numerical analysis and experiments on many standard IEEE test cases are presented, along with the comparison to the full predictor-corrector routine, confirming the efficiency of the method.

==> Shared_Settings.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\usepackage[mathscr]{euscript}
\usepackage{mdwmath}
\usepackage{bbm}
\usepackage{mathrsfs}
\usepackage{bm}
\usepackage[tight,footnotesize]{subfigure}
\usepackage{comment}
\usepackage{marginnote}
\usepackage{color}
\usepackage{tabularx}
\usepackage[flushleft]{threeparttable}
\usepackage{multirow}

\newcommand{\mydef}{:=}
\newcommand{\Rc}{\mathbb{R}}
\newcommand{\Cc}{\mathbb{C}}
\newcommand{\Nb}{N_{bus}}
\newcommand{\Ng}{N_{gen}}
\newcommand{\Nd}{N_{load}}
\newcommand{\Nl}{N_{line}}
\newcommand{\V}{\mathbf{V}}
\newcommand{\scrv}[1]{\mathit{v}_{#1}}
\newcommand{\scrw}[1]{\mathit{w}_{#1}}
\newcommand{\scrvt}[1]{\mathbf{\mathit{v}}_{#1}}
\newcommand{\scrwt}[1]{\mathbf{\mathit{w}}_{#1}}
\newcommand{\scrbt}[1]{\mathbf{\beta}_{#1}}
\newcommand{\scrth}[1]{\mathbf{\theta}_{#1}}
\newcommand{\Vv}[1]{V_{#1}}
\newcommand{\Ww}[1]{W_{#1}}
\newcommand{\cV}[1]{V^\star_{#1}}
\newcommand{\cS}[1]{S^\star_{#1}}
\newcommand{\Ss}[1]{S_{#1}}
\newcommand{\Vd}{\mathbf{V}_d}
\newcommand{\Vq}{\mathbf{V}_q}
\newcommand{\Ybus}[1]{Y_{#1}}
\newcommand{\Gg}[1]{G_{#1}} % entry of bus conductance matrix
\newcommand{\Bb}[1]{B_{#1}} % entry of bus susceptance matrix
\newcommand{\Vdq}[1]{V_{#1}} % real part and imaginary part of complex voltage [1] indicate real and imaginary part
\newcommand{\Pp}[1]{P_{#1}}
\newcommand{\Qq}[1]{Q_{#1}}
\newcommand{\U}{\mathbf{U}}
\newcommand{\M}[1]{\mathbf{M}_{#1}}
\newcommand{\Hh}[1]{\mathbf{H}_{#1}}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
\headers{Holomorphic Embedding Continuation for Power Flow}{Dan Wu and Bin Wang}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{A Holomorphic Embedding Based Continuation Method for Identifying Multiple Power Flow Solutions\thanks{Submitted to the editors DATE.
\funding{This work was partially funded by the NSF CRISP project under contract No.~1735513.}}}

% Authors: full names plus addresses.
\author{Dan Wu\thanks{Department of Mechanical Engineering, Massachusetts Institute of Technology, Cambridge, MA 
  (\email{danwumit@mit.edu}).}
\and Bin Wang\thanks{Department of Electrical and Computer Engineering, Taxes A\&M University, College Station, TX 
  (\email{binwang@tamu.edu}).}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 


==> abstract.tex <==
% REQUIRED
	\begin{abstract}
  		In this paper, we propose an efficient continuation method for locating multiple power flow solutions. We adopt the holomorphic embedding technique to derive solution curves as holomorphic functions in the form of power series for the continuation parameter. The holomorphicity of the function, which provides global information of the curve at any regular point, enables large step sizes in the path-following procedure such that non-singular curve segments can be traversed with very few steps. When approaching singular points, we switch to the traditional predictor-corrector routine to pass through them and switch back afterward to the holomorphic embedding routine. We also propose a warm starter when switching to the predictor-corrector routine, i.e. a large initial step size based on the poles of the Pad\'{e} approximation of the derived holomorphic function, since these poles reveal the locations of singularities on the curve. Numerical analysis and experiments on many standard IEEE test cases are presented, along with the comparison to the full predictor-corrector routine, confirming the efficiency of the method.
	\end{abstract}

% REQUIRED
	\begin{keywords}
  		power flow problem, holomorphic embedding, continuation
	\end{keywords}

% REQUIRED
	\begin{AMS}
  		65H10, 32A10, 14Q99 
	\end{AMS}

==> elliptic.tex <==
elliptical.
